Federated Graph Learning with Adaptive Importance-based Sampling

For privacy-preserving graph learning tasks involving distributed graph datasets, federated learning (FL)-based GCN (FedGCN) training is required. A key challenge for FedGCN is scaling to large-scale graphs, which typically incurs high computation and communication costs when dealing with the explosively increasing number of neighbors. Existing graph sampling-enhanced FedGCN training approaches ignore graph structural information or dynamics of optimization, resulting in high variance and inaccurate node embeddings. To address this limitation, we propose the Federated Adaptive Importance-based Sampling (FedAIS) approach. It achieves substantial computational cost saving by focusing the limited resources on training important nodes, while reducing communication overhead via adaptive historical embedding synchronization. The proposed adaptive importance-based sampling method jointly considers the graph structural heterogeneity and the optimization dynamics to achieve optimal trade-off between efficiency and accuracy. Extensive evaluations against five state-of-the-art baselines on five real-world graph datasets show that FedAIS achieves comparable or up to 3.23% higher test accuracy, while saving communication and computation costs by 91.77% and 85.59%.

==> history.tex <==

\subsection{Joint Analysis of Variance and Overhead} 
\label{sec:error-ana}
% \textbf{Variance reduction.} 
To construct a global FedGCN model with fast convergence speed and low prediction error, we need to first analyze the sources of variances and biases when applying graph sampling strategies. Existing graph sampling approaches suffer from high variances and biases introduced to the stochastic gradients due to the approximation of node embeddings at different layers \cite{cong2020minimal, du2022federated}. 
We denote $\tilde{h}_v^{(l)}$ as the embedding approximation of node $v\in V_k$ in the $l$-th layer. 
Specifically, the variance of stochastic gradient estimator $\tilde{g}=\sum_{k=1}^K \frac{1}{|B_k|}\sum_{v\in B_k} \nabla f(\tilde{h}_v^{(L)}, \theta_t, y_v) $, can be decomposed as: 
\begin{equation}
\label{eq:variance-decomp}
    \mathbb{E}[||\tilde{g}-\nabla F(h^{(L)}, \theta) ||]=\mathbb{E}[||\tilde{g}-g ||]+\mathbb{E}[||g-\nabla{F}(h^{(L)}, \theta)||]. 
\end{equation}
$\mathbb{E}[||\tilde{g}-g ||]$ denotes the variance of estimated gradients to their exact values $g=\sum_{k=1}^K \frac{1}{n_k}\sum_{v\in V_k} \nabla f(h_v^{(L)}, \theta_t, y_v)$, resulting from the inner layer embedding approximation in forward propagation. The term $\mathbb{E}[||g-\nabla{F}(h^{(L)}, \theta)||]$ denotes the variance of mini-batch gradients to the full gradients due to the mini-batch sampling. 
% We first make the following standard assumption on the Lipschitz continuity of the global objective function $F(h^{(L)}, \theta)$. 
\begin{assumption}
\label{ass:Lipschitz1}
    Let $F(h^{(L)}, \theta)$ be differentiable and $\lambda$-Lipschitz smooth and the value of $F(h^{(L)}, \theta)$ be bounded by a scalar $F_{inf}$. 
    % Let $A_{\theta}^{(l)}$, $U_{\theta}^{(l)}$ be Lipschitz continuous functions with Lipschitz constants $\alpha_1$, $\alpha_2$.   
\end{assumption}

% \begin{lemma}
%     Under Assumption \ref{ass:Lipschitz1}, if for all $v\in V_k$, the inputs are close to the exact inputs, i.e., $||\tilde{h}_{v}^{(l-1)}-h_{v}^{(l-1)}||\leq \beta$, the output error is bounded by:   
%     \begin{equation}
%         ||\tilde{h}_{v}^{(l)}-h_{v}^{(l)}|| \leq  (\alpha_1  |N(v)|+1)\beta \alpha_2. 
%     \end{equation}
% \end{lemma} 
% Due to the characteristics of Lipschitz constants in the function composition, we obtain the upper bound which depends on $\alpha_1$, $\alpha_2$, $|N(v)|$ and the input errors $\beta$. We then analyze the final output error.
% produced by an $L$-layer in FedGCN. 
\begin{figure}[t!]
		\centering
		\subfigure[Coauthor]{\label{fig:testAcc_bytes_illusCoauthor_CS}
	\includegraphics[width = 0.45\linewidth, height=1.18in, trim=4 4 4 4]{pictures/testAcc_bytes_illusCoauthor_CS.pdf}}
	\quad
	\subfigure[Reddit] {\label{fig:testAcc_bytes_illusReddit}
	\includegraphics[width = 0.45\linewidth, height=1.18in, trim=4 4 4 4] {pictures/testAcc_bytes_illusReddit.pdf}}
    	\vspace{-0.08in}
    	\caption{Test accuracy vs. communication cost of the FedGCN models trained on Coauthor \cite{shchur2018pitfalls} and Reddit \cite{hamilton2017inductive}.
	}
	\label{fig:testAcc_bytes_illus}
\vspace{-0.1in} 
\end{figure}


\begin{theorem}
\label{theorem:final-bound}
    Under Assumption \ref{ass:Lipschitz1}, if for all $v\in V_k$ and all $l\in \{1,2, \cdots, L-1\}$, the final output error of layer $L$ in training round $t\in [T]$ is bounded by:
\begin{equation} 
    ||\tilde{h}_{v}^{(L)}-h_{v}^{(L)}||\leq \sum_{l=1}^{L-1}\alpha_1^{L-l}\alpha_2^{L-l}|N(v)|^{L-l}. 
\end{equation}
\end{theorem} 
% Note that this upper bound does not depend on $||\tilde{h}_{v}^{(l-1)}-h_{v}^{(l-1)}||\leq \beta$. Besides, 
Theorem \ref{theorem:final-bound} lets us immediately derive an upper error bound for the estimated gradients, \emph{i.e.}, 
\begin{equation}
\label{eq:bound-gradient}
    \mathbb{E}[||\tilde{g}-g||]\leq \lambda ||\tilde{h}_v^{(L)}-h_v^{(L)}||. 
\end{equation} 

From the decomposition of variance in Eq. \eqref{eq:variance-decomp} and the upper error bound for the estimated gradients in Eq. \eqref{eq:bound-gradient}, we conclude that any graph sampling method introduces two sources of variance (\emph{i.e.}, the embedding approximation variance and the stochastic gradient variance). 
Therefore, to accelerate model convergence and reduce computation and communication overhead, both kinds of variance needs to be accounted in designing a graph sampling strategy. 

\subsection{System Overview}
\methodname{} consists of two modules (as shown in Fig. \ref{fig:system_overview}).
\begin{enumerate}
     \item \textbf{Dynamic Importance Sampling based on Historical Embeddings and Training Losses.} 
     In each training round $t$, each selected client $k$ updates the influence scores of its local training samples based on the historical embeddings and estimated training losses of individual samples. Then, each client $k$ selects its most influential node samples to be used for FedGCN model training. Using historical embeddings and training losses helps reduce both embedding approximation variance and stochastic gradient variance, thereby enabling accurate FedGCN model training. 
     % dynamically quantify samples' influence and selects nodes to compose mini-batches, where the selection probabilities are jointly calculated based on historical embeddings and estimated gradient norms. 
     % To reduce the effect of embedding approximation variance and stochastic gradient variance, we explicitly approximate node embeddings through historical embeddings acquired in previous iterations of training and 
     % we explicitly reduce it at each layer using the historical embeddings of nodes in the previous layer. 
     % in the non-synchronization iterations.
     % To save  communication costs, the local client first determines important cross-client neighbor nodes and lets the embeddings of these important cross-client neighbor nodes be transmitted for aggregation. FedAAS leverages an efficient graph attention-based influence quantification approach to iteratively and distributively update cross-neighbor selection probabilities and FedGCN models.

     % the optimization can be efficiently conducted in conjunction with gradient approximation, thus avoiding expensive calculations of 2nd-order Hessian matrices.
     \item \textbf{Adaptive Embedding Synchronization and Model Updating.} 
    With the influence estimation and sampling results, each selected  client $k$ updates its historical embeddings and performs node aggregation. Then, it updates its local model and estimates the next optimal synchronization interval via joint analysis of the overhead and error-convergence to optimize the error-runtime trade-off. Finally, client $k$ sends the updated local model to the FL server, which then aggregates the local  models to produce the global model. 
     
 \end{enumerate}
 \begin{figure}[!t]
	\begin{center}
		\includegraphics[width=0.98\linewidth,clip]{pictures/FedAIS-system.pdf}
  \vspace{-0.1in}
 		\caption{System overview of \methodname{}.  $\textcircled{1}$-$\textcircled{2}$ cross-client neighbor embeddings,     $\textcircled{3}$ local model, $\textcircled{4}$ global model $\theta_{t+1}$. }
		\vspace{-0.16in}
		\label{fig:system_overview}
	\end{center}
	%\vspace{-0.05in}
\end{figure}
\subsection{Historical Embedding-based Graph Sampling} 
% \subsection{Historical Embedding for FedGCN}  
% \label{sec:history-embed}
While evaluating embedding $h_v^{(l)}$, it is prohibitively costly to calculate all $h_v^{(l)}$ terms since they need to be computed and transmitted recursively (\emph{i.e.}, we again need the embeddings $h_w^{(l-1)}$ of all $v$'s neighbor nodes $w$). 
To reduce computation and communication costs as well as reduce the embedding approximation variance, we  introduce the historical embedding for FedGCN as an affordable approximation. 
% Our key design idea is to maintain a historical embedding $\bar{h}_{v}^{(l)}$ for each embedding $h_{v}^{(l)}$ as an affordable approximation, while saving computation and communication costs.  
% We first re-express Eq. \eqref{eq:separate} as: 
% While computing the aggregated neighbor embedding, it is prohibitively costly to evaluate all $h_v^{(l)}$ terms because they need to be computed recursively. 
% To save computation and communication overhead as well as reduce the embedding approximation variance, our key idea is to maintain a historical embedding $\bar{h}_{v}^{(l)}$ for each embedding $h_{v}^{(l)}$ as an affordable approximation. 
\begin{equation} 
\label{eq:history-calculate}
    \begin{split}
        \tilde{h}_{v}^{(l+1)}= \sigma^{(l+1)}\Big(h_{v}^{(l)}, \{h_{w}^{(l)}\}_{w\in N(v)\cap B}\cup 
        \{\bar{h}_{w}^{(l)}\}_{w\in N(v)\setminus B} \Big),\\
        \{\bar{h}_w^{(l)}\}_{w\in N(v)\setminus B}= \underbrace{\{\bar{h}_{w}^{(l)}\}_{w\in N(v)\setminus B \cap V_k}\cup 
        \{\bar{h}_{w}^{(l)}\}_{w\in N(v)\setminus V_k}}_{\text{Historical embeddings}}.  
    \end{split}
\end{equation} 

Here, we further separate the within-client neighbor nodes into two parts: 1) within-client in-batch nodes $w\in N(v)\cap B$, which are part of the current mini-batch $B_k\in V_k$; and 2) within-client out-of-batch nodes $w\in N(v)\setminus B_k \cap V_k$, which are part of the client $k$ but not included in the current mini-batch $B_k$.  
For both within-client out-of-batch nodes and cross-client neighbor nodes, we approximate their embeddings $h_w^{(l)}$ via historical embeddings $\bar{h}_w^{(l)}$ acquired in previous iterations.  
Each client maintains a storage for local historical embeddings. After each local epoch, the newly computed embeddings are pushed to the storage and serve as historical embeddings $\bar{h}_{w}^{(l)}$ for future epochs. 
The separation of in-batch nodes and out-of-batch nodes, and their approximations via historical embeddings, significantly reduces overhead as historical embeddings are retrieved from an offline storage rather than re-computed and re-transmitted. 
Compared to the previous approach which incurs exponentially higher computation and communication cost as the number of layers $L$ grows, that incurred by the proposed historical embedding-based estimator increases linearly with $L$ computation operations and communication cost per local epoch. 
% where $d^l$ is the dimension of the output $h_v^{(l)}$ of layer $l$). 
 
% We design our system to significantly reduce computation and communication costs while constructing a global model with high prediction accuracy  through the following two approaches. 
   
% as well as lower prediction errors 
% convergence speed and prediction error 


% as illustrated in Fig. \ref{fig:FedAAS-highlight}. Here, FedLocal is the federated GraghSAGE \cite{hamilton2017inductive}, which performs random selection of within-client neighbor nodes, where the cross-client neighbor node information is ignored. FedPNS performs periodic selection of cross-client neighbor nodes.  






% Threat Model: We consider the aggregator to be honest and not compromised. 

% Adversary Goal: The goal of the adversary is to manipulate the learned parameters such that the final global model M has high errors for particular classes (a subset of C). The adversary is thereby conducting a targeted poisoning attack. This differs from untargeted attacks which instead seek indiscriminate high global model errors across all classes 


 
